HAT-P-38b: A Saturn-Mass Planet Transiting a Late G Star

We report the discovery of HAT-P-38b, a Saturn-mass exoplanet transiting the V=12.56 dwarf star GSC 2314-00559 on a P = 4.6404 d circular orbit. The host star is a 0.89Msun late G-dwarf, with solar metallicity, and a radius of 0.92Rsun. The planetary companion has a mass of 0.27MJ, and radius of 0.82RJ. HAT-P-38b is one of the closest planets in mass and radius to Saturn ever discovered.

==> data/phfu_tab.tex <==
$ 55830.68887 $ & $   0.00786 $ & $   0.00085 $ & $  11.10930 $ & $ i$\\
$ 55830.69021 $ & $   0.00339 $ & $   0.00084 $ & $  11.10510 $ & $ i$\\
$ 55830.69152 $ & $   0.00650 $ & $   0.00084 $ & $  11.10810 $ & $ i$\\
$ 55830.69282 $ & $   0.00256 $ & $   0.00084 $ & $  11.10410 $ & $ i$\\
$ 55830.69414 $ & $   0.00271 $ & $   0.00084 $ & $  11.10430 $ & $ i$\\
$ 55830.69546 $ & $   0.00338 $ & $   0.00084 $ & $  11.10500 $ & $ i$\\
$ 55830.69678 $ & $   0.00228 $ & $   0.00084 $ & $  11.10360 $ & $ i$\\
$ 55830.69808 $ & $   0.00251 $ & $   0.00084 $ & $  11.10380 $ & $ i$\\
$ 55830.69939 $ & $  -0.00047 $ & $   0.00083 $ & $  11.10140 $ & $ i$\\
$ 55830.70071 $ & $   0.00058 $ & $   0.00083 $ & $  11.10240 $ & $ i$\\
$ 55830.70201 $ & $  -0.00231 $ & $   0.00083 $ & $  11.09970 $ & $ i$\\
$ 55830.70334 $ & $   0.00118 $ & $   0.00083 $ & $  11.10320 $ & $ i$\\
$ 55830.70467 $ & $   0.00082 $ & $   0.00083 $ & $  11.10220 $ & $ i$\\
$ 55830.70602 $ & $  -0.00195 $ & $   0.00082 $ & $  11.10020 $ & $ i$\\
$ 55830.70734 $ & $  -0.00168 $ & $   0.00083 $ & $  11.09990 $ & $ i$\\
$ 55830.70865 $ & $  -0.00205 $ & $   0.00083 $ & $  11.09890 $ & $ i$\\
$ 55830.70998 $ & $   0.00237 $ & $   0.00083 $ & $  11.10430 $ & $ i$\\
$ 55830.71131 $ & $   0.00124 $ & $   0.00083 $ & $  11.10250 $ & $ i$\\
$ 55830.71264 $ & $   0.00032 $ & $   0.00083 $ & $  11.10130 $ & $ i$\\
$ 55830.71395 $ & $   0.00260 $ & $   0.00083 $ & $  11.10400 $ & $ i$\\
$ 55830.71527 $ & $  -0.00025 $ & $   0.00082 $ & $  11.10110 $ & $ i$\\
$ 55830.71663 $ & $   0.00154 $ & $   0.00082 $ & $  11.10310 $ & $ i$\\
$ 55830.71795 $ & $   0.00116 $ & $   0.00082 $ & $  11.10270 $ & $ i$\\
$ 55830.71931 $ & $   0.00049 $ & $   0.00082 $ & $  11.10240 $ & $ i$\\
$ 55830.72063 $ & $   0.00048 $ & $   0.00082 $ & $  11.10260 $ & $ i$\\
$ 55830.72196 $ & $  -0.00323 $ & $   0.00082 $ & $  11.09900 $ & $ i$\\
$ 55830.72326 $ & $   0.00045 $ & $   0.00082 $ & $  11.10260 $ & $ i$\\
$ 55830.72456 $ & $  -0.00056 $ & $   0.00082 $ & $  11.10080 $ & $ i$\\
$ 55830.72587 $ & $  -0.00073 $ & $   0.00082 $ & $  11.10070 $ & $ i$\\
$ 55830.72720 $ & $   0.00126 $ & $   0.00082 $ & $  11.10280 $ & $ i$\\
$ 55830.72852 $ & $   0.00073 $ & $   0.00082 $ & $  11.10220 $ & $ i$\\
$ 55830.72983 $ & $   0.00160 $ & $   0.00082 $ & $  11.10350 $ & $ i$\\
$ 55830.73115 $ & $  -0.00042 $ & $   0.00082 $ & $  11.10160 $ & $ i$\\
$ 55830.73244 $ & $  -0.00048 $ & $   0.00081 $ & $  11.10090 $ & $ i$\\
$ 55830.73376 $ & $   0.00083 $ & $   0.00081 $ & $  11.10240 $ & $ i$\\
$ 55830.73506 $ & $  -0.00059 $ & $   0.00081 $ & $  11.10100 $ & $ i$\\
$ 55830.73638 $ & $  -0.00083 $ & $   0.00081 $ & $  11.10080 $ & $ i$\\
$ 55830.73771 $ & $  -0.00164 $ & $   0.00081 $ & $  11.10020 $ & $ i$\\
$ 55830.73903 $ & $  -0.00010 $ & $   0.00081 $ & $  11.10180 $ & $ i$\\
$ 55830.74033 $ & $  -0.00176 $ & $   0.00081 $ & $  11.10020 $ & $ i$\\
$ 55830.74166 $ & $  -0.00093 $ & $   0.00081 $ & $  11.10100 $ & $ i$\\
$ 55830.74307 $ & $   0.00004 $ & $   0.00081 $ & $  11.10210 $ & $ i$\\
$ 55830.74439 $ & $   0.00069 $ & $   0.00081 $ & $  11.10300 $ & $ i$\\
$ 55830.74572 $ & $   0.00032 $ & $   0.00081 $ & $  11.10230 $ & $ i$\\
$ 55830.74704 $ & $  -0.00007 $ & $   0.00081 $ & $  11.10170 $ & $ i$\\
$ 55830.74834 $ & $  -0.00036 $ & $   0.00080 $ & $  11.10130 $ & $ i$\\
$ 55830.74964 $ & $   0.00002 $ & $   0.00081 $ & $  11.10230 $ & $ i$\\
$ 55830.75096 $ & $  -0.00022 $ & $   0.00081 $ & $  11.10180 $ & $ i$\\
$ 55830.75228 $ & $   0.00035 $ & $   0.00080 $ & $  11.10240 $ & $ i$\\
$ 55830.75359 $ & $   0.00063 $ & $   0.00080 $ & $  11.10270 $ & $ i$\\
$ 55830.75492 $ & $  -0.00018 $ & $   0.00080 $ & $  11.10170 $ & $ i$\\
$ 55830.75625 $ & $   0.00141 $ & $   0.00080 $ & $  11.10370 $ & $ i$\\
$ 55830.75757 $ & $   0.00022 $ & $   0.00080 $ & $  11.10150 $ & $ i$\\
$ 55830.75891 $ & $  -0.00006 $ & $   0.00080 $ & $  11.10150 $ & $ i$\\
$ 55830.76022 $ & $   0.00003 $ & $   0.00081 $ & $  11.10160 $ & $ i$\\
$ 55830.76156 $ & $   0.00098 $ & $   0.00080 $ & $  11.10290 $ & $ i$\\
$ 55830.76285 $ & $   0.00020 $ & $   0.00080 $ & $  11.10270 $ & $ i$\\
$ 55830.76416 $ & $   0.00110 $ & $   0.00080 $ & $  11.10300 $ & $ i$\\
$ 55830.76548 $ & $  -0.00073 $ & $   0.00080 $ & $  11.10100 $ & $ i$\\
$ 55830.76681 $ & $   0.00095 $ & $   0.00080 $ & $  11.10300 $ & $ i$\\
$ 55830.76814 $ & $   0.00041 $ & $   0.00080 $ & $  11.10230 $ & $ i$\\
$ 55830.76951 $ & $  -0.00070 $ & $   0.00080 $ & $  11.10160 $ & $ i$\\
$ 55830.77080 $ & $  -0.00024 $ & $   0.00080 $ & $  11.10140 $ & $ i$\\
$ 55830.77211 $ & $  -0.00117 $ & $   0.00080 $ & $  11.10090 $ & $ i$\\
$ 55830.77341 $ & $  -0.00047 $ & $   0.00080 $ & $  11.10130 $ & $ i$\\
$ 55830.77473 $ & $  -0.00090 $ & $   0.00080 $ & $  11.10150 $ & $ i$\\
$ 55830.77606 $ & $  -0.00079 $ & $   0.00080 $ & $  11.10120 $ & $ i$\\
$ 55830.77737 $ & $  -0.00100 $ & $   0.00080 $ & $  11.10040 $ & $ i$\\
$ 55830.77870 $ & $  -0.00083 $ & $   0.00080 $ & $  11.10110 $ & $ i$\\
$ 55830.78001 $ & $  -0.00037 $ & $   0.00080 $ & $  11.10140 $ & $ i$\\
$ 55830.78133 $ & $  -0.00084 $ & $   0.00080 $ & $  11.10150 $ & $ i$\\
$ 55830.78264 $ & $   0.00026 $ & $   0.00080 $ & $  11.10200 $ & $ i$\\
$ 55830.78395 $ & $  -0.00179 $ & $   0.00079 $ & $  11.09970 $ & $ i$\\
$ 55830.78528 $ & $   0.00081 $ & $   0.00079 $ & $  11.10270 $ & $ i$\\
$ 55830.78662 $ & $   0.00136 $ & $   0.00079 $ & $  11.10280 $ & $ i$\\
$ 55830.78791 $ & $  -0.00020 $ & $   0.00079 $ & $  11.10170 $ & $ i$\\
$ 55830.78923 $ & $   0.00089 $ & $   0.00079 $ & $  11.10200 $ & $ i$\\
$ 55830.79056 $ & $  -0.00070 $ & $   0.00079 $ & $  11.10100 $ & $ i$\\
$ 55830.79188 $ & $   0.00126 $ & $   0.00079 $ & $  11.10250 $ & $ i$\\
$ 55830.79320 $ & $   0.00274 $ & $   0.00079 $ & $  11.10480 $ & $ i$\\
$ 55830.79453 $ & $  -0.00178 $ & $   0.00079 $ & $  11.09970 $ & $ i$\\
$ 55830.79591 $ & $   0.00082 $ & $   0.00079 $ & $  11.10250 $ & $ i$\\
$ 55830.79723 $ & $  -0.00204 $ & $   0.00079 $ & $  11.09980 $ & $ i$\\
$ 55830.79854 $ & $  -0.00315 $ & $   0.00079 $ & $  11.09840 $ & $ i$\\
$ 55830.79984 $ & $  -0.00013 $ & $   0.00079 $ & $  11.10190 $ & $ i$\\
$ 55830.80115 $ & $   0.00060 $ & $   0.00079 $ & $  11.10200 $ & $ i$\\
$ 55830.80247 $ & $   0.00004 $ & $   0.00079 $ & $  11.10110 $ & $ i$\\
$ 55830.80379 $ & $   0.00027 $ & $   0.00079 $ & $  11.10130 $ & $ i$\\
$ 55830.80511 $ & $   0.00155 $ & $   0.00079 $ & $  11.10350 $ & $ i$\\
$ 55830.80643 $ & $   0.00028 $ & $   0.00079 $ & $  11.10260 $ & $ i$\\
$ 55830.80774 $ & $   0.00041 $ & $   0.00078 $ & $  11.10220 $ & $ i$\\
$ 55830.80905 $ & $  -0.00052 $ & $   0.00079 $ & $  11.10150 $ & $ i$\\
$ 55830.81038 $ & $  -0.00036 $ & $   0.00078 $ & $  11.10210 $ & $ i$\\
$ 55830.81169 $ & $   0.00196 $ & $   0.00078 $ & $  11.10410 $ & $ i$\\
$ 55830.81302 $ & $  -0.00182 $ & $   0.00078 $ & $  11.10030 $ & $ i$\\
$ 55830.81435 $ & $   0.00119 $ & $   0.00078 $ & $  11.10350 $ & $ i$\\
$ 55830.81566 $ & $   0.00100 $ & $   0.00078 $ & $  11.10290 $ & $ i$\\
$ 55830.81696 $ & $   0.00080 $ & $   0.00078 $ & $  11.10270 $ & $ i$\\
$ 55830.81828 $ & $   0.00100 $ & $   0.00079 $ & $  11.10260 $ & $ i$\\
$ 55830.81962 $ & $   0.00030 $ & $   0.00078 $ & $  11.10190 $ & $ i$\\
$ 55830.82091 $ & $   0.00050 $ & $   0.00078 $ & $  11.10210 $ & $ i$\\
$ 55830.82238 $ & $   0.00011 $ & $   0.00078 $ & $  11.10170 $ & $ i$\\
$ 55830.82369 $ & $   0.00014 $ & $   0.00078 $ & $  11.10200 $ & $ i$\\
$ 55830.82501 $ & $   0.00090 $ & $   0.00078 $ & $  11.10230 $ & $ i$\\
$ 55830.82635 $ & $   0.00032 $ & $   0.00078 $ & $  11.10200 $ & $ i$\\
$ 55830.82766 $ & $  -0.00081 $ & $   0.00078 $ & $  11.10080 $ & $ i$\\
$ 55830.82897 $ & $  -0.00023 $ & $   0.00078 $ & $  11.10100 $ & $ i$\\
$ 55830.83027 $ & $  -0.00129 $ & $   0.00078 $ & $  11.10060 $ & $ i$\\
$ 55830.83158 $ & $   0.00114 $ & $   0.00078 $ & $  11.10280 $ & $ i$\\
$ 55830.83293 $ & $  -0.00033 $ & $   0.00078 $ & $  11.10150 $ & $ i$\\
$ 55830.83423 $ & $   0.00068 $ & $   0.00078 $ & $  11.10170 $ & $ i$\\
$ 55830.83555 $ & $  -0.00073 $ & $   0.00078 $ & $  11.10090 $ & $ i$\\
$ 55830.83687 $ & $  -0.00074 $ & $   0.00078 $ & $  11.09980 $ & $ i$\\
$ 55830.83818 $ & $  -0.00025 $ & $   0.00078 $ & $  11.10060 $ & $ i$\\
$ 55830.83949 $ & $  -0.00101 $ & $   0.00078 $ & $  11.10010 $ & $ i$\\
$ 55867.60684 $ & $   0.00215 $ & $   0.00086 $ & $  11.06770 $ & $ i$\\
$ 55867.60805 $ & $   0.00088 $ & $   0.00086 $ & $  11.06600 $ & $ i$\\
$ 55867.60925 $ & $   0.00059 $ & $   0.00086 $ & $  11.06570 $ & $ i$\\
$ 55867.61047 $ & $   0.00167 $ & $   0.00086 $ & $  11.06720 $ & $ i$\\
$ 55867.61286 $ & $  -0.00059 $ & $   0.00086 $ & $  11.06460 $ & $ i$\\
$ 55867.61409 $ & $  -0.00099 $ & $   0.00086 $ & $  11.06400 $ & $ i$\\
$ 55867.61525 $ & $  -0.00041 $ & $   0.00086 $ & $  11.06480 $ & $ i$\\
$ 55867.61647 $ & $  -0.00089 $ & $   0.00085 $ & $  11.06450 $ & $ i$\\
$ 55867.61766 $ & $   0.00085 $ & $   0.00086 $ & $  11.06590 $ & $ i$\\
$ 55867.61888 $ & $  -0.00148 $ & $   0.00085 $ & $  11.06360 $ & $ i$\\
$ 55867.62008 $ & $   0.00106 $ & $   0.00086 $ & $  11.06650 $ & $ i$\\
$ 55867.62126 $ & $  -0.00076 $ & $   0.00085 $ & $  11.06480 $ & $ i$\\
$ 55867.62248 $ & $   0.00214 $ & $   0.00085 $ & $  11.06770 $ & $ i$\\
$ 55867.62367 $ & $   0.00200 $ & $   0.00085 $ & $  11.06760 $ & $ i$\\
$ 55867.62486 $ & $  -0.00157 $ & $   0.00085 $ & $  11.06400 $ & $ i$\\
$ 55867.62606 $ & $  -0.00048 $ & $   0.00085 $ & $  11.06510 $ & $ i$\\
$ 55867.62727 $ & $  -0.00135 $ & $   0.00085 $ & $  11.06450 $ & $ i$\\
$ 55867.62848 $ & $   0.00123 $ & $   0.00085 $ & $  11.06690 $ & $ i$\\
$ 55867.62964 $ & $  -0.00060 $ & $   0.00085 $ & $  11.06520 $ & $ i$\\
$ 55867.63082 $ & $  -0.00178 $ & $   0.00085 $ & $  11.06400 $ & $ i$\\
$ 55867.63202 $ & $   0.00060 $ & $   0.00084 $ & $  11.06620 $ & $ i$\\
$ 55867.63320 $ & $  -0.00058 $ & $   0.00085 $ & $  11.06500 $ & $ i$\\
$ 55867.63440 $ & $   0.00101 $ & $   0.00084 $ & $  11.06680 $ & $ i$\\
$ 55867.63559 $ & $  -0.00127 $ & $   0.00084 $ & $  11.06450 $ & $ i$\\
$ 55867.63679 $ & $   0.00147 $ & $   0.00084 $ & $  11.06710 $ & $ i$\\
$ 55867.63800 $ & $  -0.00038 $ & $   0.00084 $ & $  11.06540 $ & $ i$\\
$ 55867.63920 $ & $   0.00061 $ & $   0.00084 $ & $  11.06690 $ & $ i$\\
$ 55867.64040 $ & $  -0.00010 $ & $   0.00084 $ & $  11.06600 $ & $ i$\\
$ 55867.64162 $ & $   0.00249 $ & $   0.00084 $ & $  11.06830 $ & $ i$\\
$ 55867.64284 $ & $   0.00055 $ & $   0.00084 $ & $  11.06660 $ & $ i$\\
$ 55867.64404 $ & $  -0.00260 $ & $   0.00084 $ & $  11.06340 $ & $ i$\\
$ 55867.64525 $ & $   0.00001 $ & $   0.00084 $ & $  11.06600 $ & $ i$\\
$ 55867.64646 $ & $   0.00073 $ & $   0.00084 $ & $  11.06670 $ & $ i$\\
$ 55867.64763 $ & $   0.00140 $ & $   0.00084 $ & $  11.06760 $ & $ i$\\
$ 55867.64882 $ & $  -0.00062 $ & $   0.00084 $ & $  11.06530 $ & $ i$\\
$ 55867.65004 $ & $  -0.00021 $ & $   0.00084 $ & $  11.06600 $ & $ i$\\
$ 55867.65123 $ & $   0.00127 $ & $   0.00084 $ & $  11.06760 $ & $ i$\\
$ 55867.65242 $ & $   0.00033 $ & $   0.00083 $ & $  11.06620 $ & $ i$\\
$ 55867.65365 $ & $   0.00091 $ & $   0.00083 $ & $  11.06700 $ & $ i$\\
$ 55867.65485 $ & $   0.00043 $ & $   0.00083 $ & $  11.06640 $ & $ i$\\
$ 55867.65604 $ & $  -0.00034 $ & $   0.00083 $ & $  11.06610 $ & $ i$\\
$ 55867.65726 $ & $  -0.00125 $ & $   0.00083 $ & $  11.06510 $ & $ i$\\
$ 55867.65845 $ & $   0.00082 $ & $   0.00083 $ & $  11.06690 $ & $ i$\\
$ 55867.65966 $ & $  -0.00045 $ & $   0.00083 $ & $  11.06610 $ & $ i$\\
$ 55867.66087 $ & $   0.00072 $ & $   0.00083 $ & $  11.06670 $ & $ i$\\
$ 55867.66205 $ & $  -0.00111 $ & $   0.00083 $ & $  11.06520 $ & $ i$\\
$ 55867.66328 $ & $  -0.00066 $ & $   0.00083 $ & $  11.06570 $ & $ i$\\
$ 55867.66447 $ & $   0.00019 $ & $   0.00083 $ & $  11.06630 $ & $ i$\\
$ 55867.66569 $ & $  -0.00020 $ & $   0.00083 $ & $  11.06560 $ & $ i$\\
$ 55867.66688 $ & $  -0.00038 $ & $   0.00082 $ & $  11.06580 $ & $ i$\\
$ 55867.66808 $ & $  -0.00310 $ & $   0.00083 $ & $  11.06330 $ & $ i$\\
$ 55867.66927 $ & $  -0.00075 $ & $   0.00082 $ & $  11.06570 $ & $ i$\\
$ 55867.67048 $ & $  -0.00076 $ & $   0.00083 $ & $  11.06530 $ & $ i$\\
$ 55867.67168 $ & $  -0.00135 $ & $   0.00083 $ & $  11.06480 $ & $ i$\\
$ 55867.67287 $ & $   0.00011 $ & $   0.00082 $ & $  11.06630 $ & $ i$\\
$ 55867.67409 $ & $  -0.00122 $ & $   0.00083 $ & $  11.06510 $ & $ i$\\
$ 55867.67527 $ & $  -0.00031 $ & $   0.00082 $ & $  11.06560 $ & $ i$\\
$ 55867.67650 $ & $  -0.00038 $ & $   0.00082 $ & $  11.06580 $ & $ i$\\
$ 55867.67765 $ & $   0.00030 $ & $   0.00082 $ & $  11.06630 $ & $ i$\\
$ 55867.67886 $ & $  -0.00184 $ & $   0.00082 $ & $  11.06460 $ & $ i$\\
$ 55867.68006 $ & $   0.00061 $ & $   0.00082 $ & $  11.06680 $ & $ i$\\
$ 55867.68126 $ & $   0.00015 $ & $   0.00082 $ & $  11.06650 $ & $ i$\\
$ 55867.68247 $ & $   0.00184 $ & $   0.00082 $ & $  11.06810 $ & $ i$\\
$ 55867.68368 $ & $   0.00048 $ & $   0.00082 $ & $  11.06680 $ & $ i$\\
$ 55867.68488 $ & $  -0.00246 $ & $   0.00082 $ & $  11.06400 $ & $ i$\\
$ 55867.68610 $ & $  -0.00043 $ & $   0.00082 $ & $  11.06600 $ & $ i$\\
$ 55867.68732 $ & $  -0.00167 $ & $   0.00082 $ & $  11.06470 $ & $ i$\\
$ 55867.68851 $ & $  -0.00141 $ & $   0.00082 $ & $  11.06510 $ & $ i$\\
$ 55867.68973 $ & $   0.00060 $ & $   0.00082 $ & $  11.06720 $ & $ i$\\
$ 55867.69092 $ & $   0.00049 $ & $   0.00082 $ & $  11.06720 $ & $ i$\\
$ 55867.69211 $ & $   0.00205 $ & $   0.00082 $ & $  11.06900 $ & $ i$\\
$ 55867.69330 $ & $   0.00179 $ & $   0.00082 $ & $  11.06890 $ & $ i$\\
$ 55867.69451 $ & $   0.00066 $ & $   0.00082 $ & $  11.06780 $ & $ i$\\
$ 55867.69572 $ & $  -0.00076 $ & $   0.00082 $ & $  11.06630 $ & $ i$\\
$ 55867.69693 $ & $  -0.00151 $ & $   0.00082 $ & $  11.06560 $ & $ i$\\
$ 55867.69813 $ & $   0.00068 $ & $   0.00082 $ & $  11.06750 $ & $ i$\\
$ 55867.69932 $ & $   0.00097 $ & $   0.00082 $ & $  11.06790 $ & $ i$\\
$ 55867.70052 $ & $   0.00156 $ & $   0.00082 $ & $  11.06870 $ & $ i$\\
$ 55867.70173 $ & $   0.00193 $ & $   0.00081 $ & $  11.06890 $ & $ i$\\
$ 55867.70294 $ & $   0.00395 $ & $   0.00082 $ & $  11.07100 $ & $ i$\\
$ 55867.70414 $ & $   0.00586 $ & $   0.00082 $ & $  11.07280 $ & $ i$\\
$ 55867.70534 $ & $   0.00592 $ & $   0.00082 $ & $  11.07280 $ & $ i$\\
$ 55867.70653 $ & $   0.00457 $ & $   0.00082 $ & $  11.07170 $ & $ i$\\
$ 55867.70775 $ & $   0.00678 $ & $   0.00082 $ & $  11.07390 $ & $ i$\\
$ 55867.70894 $ & $   0.00757 $ & $   0.00082 $ & $  11.07470 $ & $ i$\\
$ 55867.71015 $ & $   0.00758 $ & $   0.00082 $ & $  11.07450 $ & $ i$\\
$ 55867.71133 $ & $   0.00873 $ & $   0.00082 $ & $  11.07570 $ & $ i$\\
$ 55867.71253 $ & $   0.00896 $ & $   0.00082 $ & $  11.07600 $ & $ i$\\
$ 55867.71373 $ & $   0.00748 $ & $   0.00082 $ & $  11.07450 $ & $ i$\\
$ 55867.71495 $ & $   0.00816 $ & $   0.00082 $ & $  11.07480 $ & $ i$\\
$ 55867.71614 $ & $   0.00943 $ & $   0.00082 $ & $  11.07660 $ & $ i$\\
$ 55867.71733 $ & $   0.00935 $ & $   0.00082 $ & $  11.07650 $ & $ i$\\
$ 55867.71852 $ & $   0.00913 $ & $   0.00082 $ & $  11.07610 $ & $ i$\\
$ 55867.71973 $ & $   0.01054 $ & $   0.00082 $ & $  11.07760 $ & $ i$\\
$ 55867.72091 $ & $   0.01017 $ & $   0.00082 $ & $  11.07720 $ & $ i$\\
$ 55867.72212 $ & $   0.00980 $ & $   0.00082 $ & $  11.07700 $ & $ i$\\
$ 55867.72333 $ & $   0.00953 $ & $   0.00082 $ & $  11.07670 $ & $ i$\\
$ 55867.72451 $ & $   0.00960 $ & $   0.00082 $ & $  11.07680 $ & $ i$\\
$ 55867.72570 $ & $   0.00991 $ & $   0.00082 $ & $  11.07720 $ & $ i$\\
$ 55867.72689 $ & $   0.00986 $ & $   0.00082 $ & $  11.07720 $ & $ i$\\
$ 55867.72811 $ & $   0.00723 $ & $   0.00082 $ & $  11.07480 $ & $ i$\\
$ 55867.72930 $ & $   0.00984 $ & $   0.00082 $ & $  11.07700 $ & $ i$\\
$ 55867.73051 $ & $   0.01028 $ & $   0.00082 $ & $  11.07740 $ & $ i$\\
$ 55867.73169 $ & $   0.01109 $ & $   0.00082 $ & $  11.07840 $ & $ i$\\
$ 55867.73289 $ & $   0.01000 $ & $   0.00082 $ & $  11.07700 $ & $ i$\\
$ 55867.73408 $ & $   0.01004 $ & $   0.00082 $ & $  11.07720 $ & $ i$\\
$ 55867.73528 $ & $   0.01061 $ & $   0.00081 $ & $  11.07770 $ & $ i$\\
$ 55867.73647 $ & $   0.01218 $ & $   0.00082 $ & $  11.07950 $ & $ i$\\
$ 55867.73765 $ & $   0.00949 $ & $   0.00081 $ & $  11.07670 $ & $ i$\\
$ 55867.73885 $ & $   0.01132 $ & $   0.00082 $ & $  11.07890 $ & $ i$\\
$ 55867.74002 $ & $   0.01106 $ & $   0.00082 $ & $  11.07860 $ & $ i$\\
$ 55867.74120 $ & $   0.00846 $ & $   0.00081 $ & $  11.07610 $ & $ i$\\
$ 55867.74239 $ & $   0.00984 $ & $   0.00081 $ & $  11.07740 $ & $ i$\\
$ 55867.74359 $ & $   0.01173 $ & $   0.00082 $ & $  11.07940 $ & $ i$\\
$ 55867.74504 $ & $   0.01039 $ & $   0.00081 $ & $  11.07810 $ & $ i$\\
$ 55867.74631 $ & $   0.00913 $ & $   0.00081 $ & $  11.07660 $ & $ i$\\
$ 55867.74748 $ & $   0.01139 $ & $   0.00082 $ & $  11.07880 $ & $ i$\\
$ 55867.74877 $ & $   0.01098 $ & $   0.00082 $ & $  11.07840 $ & $ i$\\
$ 55867.75019 $ & $   0.01118 $ & $   0.00082 $ & $  11.07890 $ & $ i$\\
$ 55867.75149 $ & $   0.01091 $ & $   0.00082 $ & $  11.07830 $ & $ i$\\
$ 55867.75268 $ & $   0.01171 $ & $   0.00082 $ & $  11.07880 $ & $ i$\\
$ 55867.75389 $ & $   0.01034 $ & $   0.00081 $ & $  11.07770 $ & $ i$\\
$ 55867.75506 $ & $   0.01077 $ & $   0.00081 $ & $  11.07790 $ & $ i$\\
$ 55867.75627 $ & $   0.01101 $ & $   0.00081 $ & $  11.07840 $ & $ i$\\
$ 55867.75749 $ & $   0.01220 $ & $   0.00081 $ & $  11.07960 $ & $ i$\\
$ 55867.75871 $ & $   0.01216 $ & $   0.00081 $ & $  11.07940 $ & $ i$\\
$ 55867.75988 $ & $   0.01077 $ & $   0.00081 $ & $  11.07810 $ & $ i$\\
$ 55867.76108 $ & $   0.01033 $ & $   0.00081 $ & $  11.07790 $ & $ i$\\
$ 55867.76227 $ & $   0.01089 $ & $   0.00081 $ & $  11.07830 $ & $ i$\\
$ 55867.76349 $ & $   0.00871 $ & $   0.00081 $ & $  11.07630 $ & $ i$\\
$ 55867.76469 $ & $   0.01060 $ & $   0.00081 $ & $  11.07790 $ & $ i$\\
$ 55867.76590 $ & $   0.01135 $ & $   0.00081 $ & $  11.07890 $ & $ i$\\
$ 55867.76710 $ & $   0.00974 $ & $   0.00081 $ & $  11.07720 $ & $ i$\\
$ 55867.76829 $ & $   0.01074 $ & $   0.00081 $ & $  11.07820 $ & $ i$\\
$ 55867.76949 $ & $   0.00936 $ & $   0.00081 $ & $  11.07710 $ & $ i$\\
$ 55867.77071 $ & $   0.00966 $ & $   0.00081 $ & $  11.07760 $ & $ i$\\
$ 55867.77190 $ & $   0.01129 $ & $   0.00081 $ & $  11.07900 $ & $ i$\\
$ 55867.77312 $ & $   0.00993 $ & $   0.00081 $ & $  11.07740 $ & $ i$\\
$ 55867.77429 $ & $   0.00910 $ & $   0.00081 $ & $  11.07680 $ & $ i$\\
$ 55867.77550 $ & $   0.00978 $ & $   0.00081 $ & $  11.07740 $ & $ i$\\
$ 55867.77671 $ & $   0.01188 $ & $   0.00081 $ & $  11.07940 $ & $ i$\\
$ 55867.77791 $ & $   0.00940 $ & $   0.00081 $ & $  11.07700 $ & $ i$\\
$ 55867.77910 $ & $   0.00982 $ & $   0.00081 $ & $  11.07730 $ & $ i$\\
$ 55867.78028 $ & $   0.01129 $ & $   0.00081 $ & $  11.07880 $ & $ i$\\
$ 55867.78150 $ & $   0.01046 $ & $   0.00081 $ & $  11.07790 $ & $ i$\\
$ 55867.78270 $ & $   0.00938 $ & $   0.00081 $ & $  11.07710 $ & $ i$\\
$ 55867.78388 $ & $   0.00828 $ & $   0.00081 $ & $  11.07590 $ & $ i$\\
$ 55867.78508 $ & $   0.01120 $ & $   0.00081 $ & $  11.07900 $ & $ i$\\
$ 55867.78629 $ & $   0.00916 $ & $   0.00081 $ & $  11.07700 $ & $ i$\\
$ 55867.78753 $ & $   0.01057 $ & $   0.00081 $ & $  11.07840 $ & $ i$\\
$ 55867.78873 $ & $   0.01102 $ & $   0.00081 $ & $  11.07890 $ & $ i$\\
$ 55867.78995 $ & $   0.01061 $ & $   0.00081 $ & $  11.07850 $ & $ i$\\
$ 55867.79114 $ & $   0.00939 $ & $   0.00081 $ & $  11.07710 $ & $ i$\\
$ 55867.79234 $ & $   0.01143 $ & $   0.00081 $ & $  11.07920 $ & $ i$\\
$ 55867.79352 $ & $   0.01052 $ & $   0.00081 $ & $  11.07820 $ & $ i$\\
$ 55867.79473 $ & $   0.01105 $ & $   0.00081 $ & $  11.07890 $ & $ i$\\
$ 55867.79594 $ & $   0.00769 $ & $   0.00081 $ & $  11.07530 $ & $ i$\\
$ 55867.80068 $ & $   0.01014 $ & $   0.00081 $ & $  11.07780 $ & $ i$\\
$ 55867.80183 $ & $   0.00901 $ & $   0.00081 $ & $  11.07680 $ & $ i$\\
$ 55867.80306 $ & $   0.00965 $ & $   0.00081 $ & $  11.07760 $ & $ i$\\
$ 55867.80425 $ & $   0.00973 $ & $   0.00081 $ & $  11.07770 $ & $ i$\\
$ 55867.80546 $ & $   0.00896 $ & $   0.00081 $ & $  11.07730 $ & $ i$\\
$ 55867.80666 $ & $   0.00747 $ & $   0.00080 $ & $  11.07590 $ & $ i$\\
$ 55867.80786 $ & $   0.00767 $ & $   0.00081 $ & $  11.07610 $ & $ i$\\
$ 55867.80905 $ & $   0.00886 $ & $   0.00081 $ & $  11.07730 $ & $ i$\\
$ 55867.81025 $ & $   0.00821 $ & $   0.00081 $ & $  11.07600 $ & $ i$\\
$ 55867.81145 $ & $   0.00738 $ & $   0.00081 $ & $  11.07540 $ & $ i$\\
$ 55867.81265 $ & $   0.00738 $ & $   0.00081 $ & $  11.07540 $ & $ i$\\
$ 55867.81386 $ & $   0.00793 $ & $   0.00081 $ & $  11.07580 $ & $ i$\\
$ 55867.81505 $ & $   0.00461 $ & $   0.00081 $ & $  11.07260 $ & $ i$\\
$ 55867.81625 $ & $   0.00418 $ & $   0.00081 $ & $  11.07200 $ & $ i$\\
$ 55867.81748 $ & $   0.00212 $ & $   0.00081 $ & $  11.06970 $ & $ i$\\
$ 55867.81867 $ & $   0.00082 $ & $   0.00081 $ & $  11.06830 $ & $ i$\\
$ 55867.81988 $ & $   0.00064 $ & $   0.00080 $ & $  11.06810 $ & $ i$\\
$ 55867.82106 $ & $   0.00118 $ & $   0.00081 $ & $  11.06850 $ & $ i$\\
$ 55867.82226 $ & $  -0.00040 $ & $   0.00081 $ & $  11.06700 $ & $ i$\\
$ 55867.82345 $ & $  -0.00004 $ & $   0.00080 $ & $  11.06740 $ & $ i$\\
$ 55867.82467 $ & $   0.00033 $ & $   0.00081 $ & $  11.06770 $ & $ i$\\
$ 55867.82587 $ & $  -0.00005 $ & $   0.00080 $ & $  11.06730 $ & $ i$\\
$ 55867.82704 $ & $   0.00195 $ & $   0.00080 $ & $  11.06950 $ & $ i$\\
$ 55867.82826 $ & $   0.00215 $ & $   0.00081 $ & $  11.06940 $ & $ i$\\
$ 55867.82945 $ & $   0.00243 $ & $   0.00081 $ & $  11.07010 $ & $ i$\\
$ 55867.83066 $ & $   0.00106 $ & $   0.00080 $ & $  11.06820 $ & $ i$\\
$ 55867.83189 $ & $  -0.00002 $ & $   0.00081 $ & $  11.06730 $ & $ i$\\
$ 55867.83308 $ & $   0.00053 $ & $   0.00081 $ & $  11.06810 $ & $ i$\\
$ 55867.83430 $ & $  -0.00107 $ & $   0.00080 $ & $  11.06640 $ & $ i$\\
$ 55867.83550 $ & $  -0.00016 $ & $   0.00080 $ & $  11.06700 $ & $ i$\\
$ 55867.83671 $ & $   0.00047 $ & $   0.00081 $ & $  11.06770 $ & $ i$\\
$ 55867.83789 $ & $  -0.00006 $ & $   0.00081 $ & $  11.06710 $ & $ i$\\
$ 55867.83915 $ & $   0.00061 $ & $   0.00080 $ & $  11.06790 $ & $ i$\\
$ 55867.84063 $ & $  -0.00058 $ & $   0.00080 $ & $  11.06700 $ & $ i$\\
$ 55867.84183 $ & $   0.00023 $ & $   0.00081 $ & $  11.06740 $ & $ i$\\
$ 55867.84305 $ & $   0.00060 $ & $   0.00081 $ & $  11.06810 $ & $ i$\\
$ 55867.84426 $ & $   0.00122 $ & $   0.00081 $ & $  11.06870 $ & $ i$\\
$ 55867.84557 $ & $   0.00046 $ & $   0.00081 $ & $  11.06790 $ & $ i$\\
$ 55867.84698 $ & $   0.00011 $ & $   0.00081 $ & $  11.06760 $ & $ i$\\
$ 55867.84834 $ & $   0.00099 $ & $   0.00081 $ & $  11.06840 $ & $ i$\\
$ 55867.84954 $ & $   0.00038 $ & $   0.00080 $ & $  11.06750 $ & $ i$\\
$ 55867.85073 $ & $  -0.00041 $ & $   0.00081 $ & $  11.06720 $ & $ i$\\
$ 55867.85191 $ & $  -0.00050 $ & $   0.00081 $ & $  11.06700 $ & $ i$\\
$ 55867.85311 $ & $  -0.00040 $ & $   0.00081 $ & $  11.06700 $ & $ i$\\
$ 55867.85430 $ & $   0.00018 $ & $   0.00081 $ & $  11.06730 $ & $ i$\\
$ 55867.85551 $ & $   0.00026 $ & $   0.00081 $ & $  11.06740 $ & $ i$\\
$ 55867.85673 $ & $   0.00070 $ & $   0.00081 $ & $  11.06790 $ & $ i$\\
$ 55867.85797 $ & $   0.00022 $ & $   0.00081 $ & $  11.06750 $ & $ i$\\
$ 55867.85916 $ & $  -0.00197 $ & $   0.00081 $ & $  11.06540 $ & $ i$\\
$ 55867.86036 $ & $  -0.00083 $ & $   0.00081 $ & $  11.06640 $ & $ i$\\
$ 55867.86154 $ & $   0.00121 $ & $   0.00081 $ & $  11.06860 $ & $ i$\\
$ 55867.86275 $ & $  -0.00168 $ & $   0.00081 $ & $  11.06560 $ & $ i$\\
$ 55867.86394 $ & $  -0.00002 $ & $   0.00081 $ & $  11.06740 $ & $ i$\\
$ 55867.86514 $ & $   0.00077 $ & $   0.00081 $ & $  11.06810 $ & $ i$\\
$ 55867.86633 $ & $  -0.00075 $ & $   0.00081 $ & $  11.06630 $ & $ i$\\
$ 55867.86750 $ & $  -0.00058 $ & $   0.00081 $ & $  11.06680 $ & $ i$\\
$ 55867.86871 $ & $  -0.00104 $ & $   0.00081 $ & $  11.06640 $ & $ i$\\
$ 55867.86990 $ & $  -0.00031 $ & $   0.00081 $ & $  11.06690 $ & $ i$\\
$ 55867.87110 $ & $   0.00029 $ & $   0.00081 $ & $  11.06750 $ & $ i$\\
$ 55867.87233 $ & $  -0.00047 $ & $   0.00081 $ & $  11.06710 $ & $ i$\\
$ 55867.87351 $ & $   0.00134 $ & $   0.00081 $ & $  11.06870 $ & $ i$\\
$ 55867.87473 $ & $   0.00054 $ & $   0.00081 $ & $  11.06810 $ & $ i$\\
$ 55867.87593 $ & $  -0.00079 $ & $   0.00081 $ & $  11.06640 $ & $ i$\\
$ 55867.87713 $ & $  -0.00095 $ & $   0.00081 $ & $  11.06660 $ & $ i$\\
$ 55867.87835 $ & $  -0.00182 $ & $   0.00081 $ & $  11.06540 $ & $ i$\\
$ 55867.87953 $ & $  -0.00112 $ & $   0.00081 $ & $  11.06590 $ & $ i$\\
$ 55867.88073 $ & $  -0.00015 $ & $   0.00081 $ & $  11.06690 $ & $ i$\\

